Scaling Properties of Deep Residual Networks

Residual networks (ResNets) have displayed impressive results in pattern recognition and, recently, have garnered considerable theoretical interest due to a perceived link with neural ordinary differential equations (neural ODEs). This link relies on the convergence of network weights to a smooth function as the number of layers increases. We investigate the properties of weights trained by stochastic gradient descent and their scaling with network depth through detailed numerical experiments. We observe the existence of scaling regimes markedly different from those assumed in neural ODE literature. Depending on certain features of the network architecture, such as the smoothness of the activation function, one may obtain an alternative ODE limit, a stochastic differential equation or neither of these. These findings cast doubts on the validity of the neural ODE model as an adequate asymptotic description of deep ResNets and point to an alternative class of differential equations as a better description of the deep network limit.

==> sec/camera-ready/notes.tex <==

DONE
\begin{itemize}
    \item DONE - Put a picture for $A_k$ (look like white noise) for the  ReLU case in Figure 1 and then motivate the sum (which may not seem to be nature for the readers at the beginning) -> between the two Figures in Section 2. 
    \item $\alpha=1$ and $\beta=0$ is the Neural ODE limit (Chen, Thrope)
    \item DONE - Updates computations for beta
    \item DONE - Updates figures accordingly
    \item DONE Add hyperparameters sensitivity table in the appendix
    \item DONE - add remark on relevance of the different norms under Hyp 1 + 2
    \item DONE - modify the link to the experiments
    \item DONE - Add more literature review as in Alain's slides.
    \item DONE put the 3 figures in one column mode
    \item DONE Reduce the cases in Section 4 (only $\gamma=1/2$).
    \item Explain remark 2.1 more: in particular, explain the (fair) comment from Reviewer 5 saying that $A^{(L)}_k = A^{(2L)}_k + A^{(2L)}_{k+1}$ is actually enforced by Remark 2.1, which might sound a little bit odd
\end{itemize}

TO DO
\begin{itemize}
    \item Add insights for training deep networks
    \item When explaining the numerical results, link and comment more with the Neural ODE (put a remark in Section 4)
    \item Rework formulation of the results
\item   Literature review: ResNet and Neural ODE
\end{itemize}



Q: Shall we put here a wishy-washy argument saying that since Hyp 2 is satisfied at init, and we update the weights using gradients of a $C^1$ by part functional, we would expect Hyp 2 to remain true along training (and we test for that) \\


